Measuring Human Perception to Improve Open Set Recognition

The human ability to recognize when an object belongs or does not belong to a particular vision task outperforms all open set recognition algorithms. Human perception as measured by the methods and procedures of visual psychophysics from psychology provides an additional data stream for algorithms that need to manage novelty. For instance, measured reaction time from human subjects can offer insight as to whether a class sample is prone to be confused with a different class -- known or novel. In this work, we designed and performed a large-scale behavioral experiment that collected over 200,000 human reaction time measurements associated with object recognition. The data collected indicated reaction time varies meaningfully across objects at the sample-level. We therefore designed a new psychophysical loss function that enforces consistency with human behavior in deep networks which exhibit variable reaction time for different images. As in biological vision, this approach allows us to achieve good open set recognition performance in regimes with limited labeled training data. Through experiments using data from ImageNet, significant improvement is observed when training Multi-Scale DenseNets with this new formulation: it significantly improved top-1 validation accuracy by 6.02%, top-1 test accuracy on known samples by 9.81%, and top-1 test accuracy on unknown samples by 33.18%. We compared our method to 10 open set recognition methods from the literature, which were all outperformed on multiple metrics.

==> Arxiv submission file/README <==

August 26, 2015


IEEEtran is a LaTeX class for authors of the Institute of Electrical and
Electronics Engineers (IEEE) transactions journals and conferences.
The latest version of the IEEEtran package can be found at CTAN:

http://www.ctan.org/pkg/ieeetran

as well as within IEEE's site:

http://www.ieee.org/


This package contains the IEEE Computer Society subset of the full IEEEtran
package and is intended for use with IEEE Computer Society publications.
The included version of the IEEEtran_HOWTO.pdf has been specially formatted
in IEEE Computer Society (compsoc) journal mode.


For latest news, helpful tips, answers to frequently asked questions,
beta releases and other support, visit the IEEEtran home page at my
website:

http://www.michaelshell.org/tex/ieeetran/

Version 1.8b has a number of significant changes over the v1.8a release.
For a full history of changes, please read the file changelog.txt.
The most notable changes in this release include:

 1) Added new comsoc mode for the IEEE Communications Society.
    This mode (at present) only invokes the use of the newtxmath math fonts.
 
 2) Revised IEEEeqnarray column specifications to work with active " 
    (or other punctuation catcode changes) as with babel under the
    german or ngerman language modes. 
    Thanks to Stefan M. Moser for reporting this problem.

 3) Added \indexspace and other index related macros as newer versions of
    article.cls now do. These macros are needed to avoid an error when
    using the glossaries package.
    Thanks to Sebastian Nyberg for suggesting this change.

 4) Fixed odd/even page header font bug under compsoc mode and
    other page style code improvements.
    Thanks to Marco Paolieri for reporting this problem.

 5) Added hooks to allow for easy control of spacing above title.

 6) Added the \IEEEnoauxwrite command.
    Thanks to Sudarshan Mukherjee for suggesting this feature.


NOTE: Take care not to confuse the "comsoc" and "compsoc" class
options/modes as they are very different:

comsoc  ==> IEEE Communications Society
compsoc ==> IEEE Computer Society

The comsoc mode requires that an acceptable Times math font be available on
the LaTeX system. This requirement will be enforced by IEEEtran in comsoc
mode. Either the freely available newtxmath font by Michael Sharpe
http://www.ctan.org/pkg/newtx
(version 1.451, July 28, 2015 or later is recommended)
or the commercial MathTime font (e.g., mtpro2.sty) is acceptable.
See Section II-D (2.4) "Class Options - comsoc, compsoc, transmag" of
the IEEEtran HOWTO for more details.


Best wishes for all your publication endeavors,

Michael Shell
http://www.michaelshell.org/


********************************** Files **********************************

README                 - This file.

IEEEtran.cls           - The IEEEtran LaTeX class file.

changelog.txt          - The revision history.

IEEEtran_HOWTO.pdf     - The IEEEtran LaTeX class user manual.

bare_conf_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         conference papers.

bare_jrnl_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         journal papers.

bare_adv.tex           - A bare bones starter file showing advanced
                         techniques such as conditional compilation,
                         hyperlinks, PDF thumbnails, etc. The illustrated
                         format is for a IEEE Computer Society journal paper.

***************************************************************************
Legal Notice:
This code is offered as-is without any warranty either expressed or
implied; without even the implied warranty of MERCHANTABILITY or
FITNESS FOR A PARTICULAR PURPOSE! 
User assumes all risk.
In no event shall the IEEE or any contributor to this code be liable for
any damages or losses, including, but not limited to, incidental,
consequential, or any other damages, resulting from the use or misuse
of any information contained here.

All comments are the opinions of their respective authors and are not
necessarily endorsed by the IEEE.

This work is distributed under the LaTeX Project Public License (LPPL)
( http://www.latex-project.org/ ) version 1.3, and may be freely used,
distributed and modified. A copy of the LPPL, version 1.3, is included
in the base LaTeX documentation of all distributions of LaTeX released
2003/12/01 or later.
Retain all contribution notices and credits.
** Modified files should be clearly indicated as such, including  **
** renaming them and changing author support contact information. **

File list of work: IEEEtran.cls, IEEEtran_HOWTO.pdf, bare_adv.tex,
                   bare_conf_compsoc.tex, bare_jrnl_compsoc.tex.
***************************************************************************


==> Arxiv submission file/sections/a_intro.tex <==
\section{Introduction}
Open Set Recognition (OSR) is a task that is extremely challenging for computer vision algorithms~\cite{geng2020recent}, but something that can be effortlessly performed by humans without the need for very large labeled datasets~\cite{sunday2021novel}. In machine learning-based computer vision, OSR is defined as novelty detection coupled with closed set classification, where novelties are visual information not seen at training time that should not inhibit classification performance~\cite{walter_open_set}. At the class level, images from classes that are seen in both the training and testing phases are called known classes, while those that are not seen in training and only encountered in testing are considered to be unknown classes (\textit{i.e.}, novel classes). 

While some existing systems can detect unknown classes based on previous known knowledge~\cite{geng2020recent}, humans can not only recognize unknown instances but also avoid the under-generalization problem machine learning models face when fitting to known class data using just supervised labels~\cite{tenenbaum2011grow}. Psychologists study this phenomenon by using the methods and procedures of visual psychophysics to measure the human behavior associated with a particular task~\cite{lu2013visual}. Reaction time (RT) is one of the most diagnostic measurable behaviors because it reveals patterns of difficulty in the data (\textit{e.g.}, it is fast to recognize something that is familiar, while more ambiguous cases will take longer to be recognized).

\begin{figure}[t]
    \centering
    \includegraphics[width=\linewidth]{fig/teaser_4imgs_revision_gs.pdf}
    \caption{In this work, we conduct behavioral experiments to gauge the human perception of objects that belong or don't belong to a task. Through the use of visual psychophysics, human reaction time is measured across tasks (top panel). These measurements are then used in a novel psychophysical loss function to train biologically-inspired deep networks with a variable reaction time property, leading to better novelty detection and multi-class classification performance in open set recognition settings (bottom panel).
    }
    \label{fig:teaser}
    \vspace{-5mm}
\end{figure}

In this paper, we consider the possibility of incorporating measurements of human reaction time into the OSR process to improve model performance. The subtleties of human perception measured by psychophysics methods have already made in-roads in other computer vision tasks~\cite{Scheirer_2014_TPAMI,mccurrie2017predicting,grieggs2020measuring}, making this strategy an attractive target for OSR.
The fact that humans can separate objects that belong to a task from objects that do not in a better way than machines indicates that incorporating psychophysical measurements of human reaction time into the model training process may provide more information to learn from, and thus better performance.
The challenge is in designing a biologically-inspired neural network architecture with its own variable reaction time and conditioning it to match human behavior as closely as possible. 

% Introduce our work - method in general
The first step to solving this problem is collecting data that are useful in the context of novelty management.
Boult et al.~\cite{boult2020unifying} have recently argued that much of the existing OSR work consists of ill-defined novelty problems, making both data collection and algorithm design more difficult than is necessary. Thus they introduce a formal taxonomy of novelty and suggest that the perception of novelty can be decoupled from the ``ground-truth'' novelty value of objects in the environment. This means that something can be novel to an agent (artificial or human) that may not be truly novel in the environment (\textit{i.e.}, it has not been learned yet). In-line with this, we designed a human behavioral experiment which gauged the human perception of class-level information via reaction time measurement (Fig.~\ref{fig:teaser}, top panel). We collected over 200,000 psychophysical reaction time measurements using this experiment design for a partition of ImageNet containing 335 total classes~\cite{UMD_dataset}. Compared to prior work in OSR~\cite{Bendale_2016_CVPR,Rudd_2018,zhou2021learning,crosr,cacosr}, this dataset is far more realistic and challenging than the open set partitions of MNIST, SVNH, CIFAR10 and other small datasets that are commonly found in the literature. But it is intentionally more limited in available training images compared to the common ImageNet-based OSR training regimes.

The second step is the formulation of the machine learning strategy. After obtaining knowledge of the correlation between reaction time and OSR performance for individual images, we designed a new psychophysical loss function that can enforce more consistent behavior between humans and machines when training a deep neural network, thus improving the performance on OSR problems (Fig.~\ref{fig:teaser}, bottom panel).
To ensure the best match between the newly introduced loss function and the task, we chose to use the Multi-Scale DenseNet~\cite{huang2018multiscale} (MSD-Net) architecture as a proof-of-concept.
MSD-Net has five classifiers at different depths in its architecture, making it possible to measure model reaction time by observing the classifier that serves as the exit point for a particular image.
We believe that coupling large-scale psychophysically annotated data with a loss function that makes use of behavioral measurements like reaction time to induce similar behavior in models is a viable path forward for the OSR problem. 

% Evaluation results
%\textcolor{red}{(is there anything to cite for this imageNet sub-set??)}
%The method is majorly evaluated by %training MSD-Net on a subset of %ImageNet~\cite{deng2009imagenet} with %the newly introduced psychophysical %loss. The best model obtained when %training with the psychophysical loss %improved top-1 validation accuracy by %7\%, top-1 accuracy on test known %classes by 18\% and test accuracy on %unknown class by 33\%, comparing to a %baseline method trained with the %standard Cross-Entropy loss and tested %with simple thresholding. Besides, we %also accomplish experiments for other 9 %baseline methods on our dataset, and %show our method significantly %outperforms all of them using multiple %metrics. We observe that some previous %methods fail on the task using our %dataset by either classifying all the %samples as known or all as unknown.

% Bullet points - list our contributions
\textbf{In summary, the major contributions of this paper are:} \textbf{(1)} 
A new dataset for the OSR problem containing reaction time measurements for a challenging partition of ImageNet.
This data is analyzed to draw out patterns of difficulty not evident from the original class-level labels.
This is the first large-scale human behavior study carried out to explore the use of psychophysical measurements for OSR, and it provides a wealth of data for other researchers working on this problem and related ones\footnote{All data and code will be released after publication.}.
\textbf{(2)} A general strategy for utilizing measured human reaction time for training deep networks for OSR, implemented as a psychophysical loss function that can improve the performance of any neural network architecture that supports variable reaction times for different inputs.
\textbf{(3)} A specific implementation of the loss strategy that takes advantage of the special structure of the MSD-Net architecture.
\textbf{(4)} Extensive experimentation over the OSR partition of ImageNet that balances class diversity and limited training data, with comparison made to 10 recent OSR approaches from the literature.
MSD-Net models that are trained with the proposed psychophysical loss function are shown to significantly outperform prior work. 

==> Arxiv submission file/sections/b_related_work.tex <==
\section{Related Work}

%Work on novelty detection, Open-Set %Recognition and specific studies of human %perception related to it can be found in many %disciplines. In this section, we review some %of the previous work that is aligned with this %topic to put our work in context.

%\subsection{Recent Advance in Novelty Detection}
%\textcolor{red}{Do we need this section? We %did not compare with or use any of these %methods. We need to draw a connection %between this and OSR.}

%Novelty detection can be defined as distinguishing the test data that is different from training data in some aspect. Originally, novelty detection was considered to be equivalent to \textit{one-class classification}\cite{one_class}, where the known samples are supposed to be classified into a single class, while unknown samples should be distinguished from non-novel samples as another class. Two synonyms for novelty detection that can be found in the literature are \textit{anomaly detection}\cite{10.1145/1541880.1541882} and \textit{outlier detection} \cite{RITTER1997525}. The challenging nature of novelty detection and the necessity for studying it for many domains has been drawing it much attention in recent years.

%Researchers have been exploring methods for novelty detection since the early days of statistical pattern recognition. As there exists an enormous number of methods for novelty detection, several surveys~\cite{MARKOU20032481, MARKOU20032499,10.1007/978-3-642-17080-5_21, 4017846, OutlierDetection, outlier-mining} have reviewed these methods and classified them into different branches, and a very recent and thorough review~\cite{PIMENTEL2014215} classifies them into five general categories: (1) Probabilistic methods \cite{doi:10.1080/00401706.1969.10490657, 4216858, Hazan2012ExtremeVS} usually estimate the probability dense functions (PDF) of a distribution, and then certain thresholds are applied to distinguish novel and non-novel samples. (2) Distance-based methods, including clustering \cite{Barbar2002COOLCATAE, 5415638} and nearest-neighbor \cite{1334558, 7ddea41e0abc45bba36f8bc345e31bf4, 10.1007/3-540-45681-3_2}, aim at building well-defined distance functions to compute the distance between points. (3) Reconstruction-based methods are normally used in safety-critical applications. Neural network based methods \cite{doi:10.1080/01431160110055804, 1014330, 1184035} and sub-space based methods \cite{6133296, Gnter2007FastIK} are two most popular sub-categories under this branch. (4) Domain-base methods \cite{NIPS2000_0e087ec5, 5596456, 10.1007/11760191_122, Evangelista2004TamingTC} create a boundary based on the structure of the training dataset; they are designed to describe a \textit{domain} instead of a \textit{class}, and are typically insensitive to the specific sampling and density. (5) Information-theoretic techniques \cite{DBLP:journals/corr/abs-cs-0503081, DBLP:journals/corr/abs-cs-0507065, 4470225} compute the information content of a dataset, and they assume the information contained by novel samples vary largely from those non-novel samples. 

% One paragraph for SAIL-ON and theory
%Although much work has been done in general novelty detection, there is no universally agreed definition for ``novelty", and most work usually define their novelty in different ways according to the method they are designing or the application they are working on. To address the problem arise from ill-defined novelty problems, Boult et al. \cite{boult2020unifying} first propose a unified framework to formalize the theories of novelty. In their paper, the authors emphasize the importance of defining "what is novel" when designing AI agents, and present frameworks for formalizing novelty for static or learning-based agents; the work focuses on evaluating whether an input is novel when given to an agents, instead of generating novelties.

\textbf{Open Set Recognition.} The development of capabilities that can detect that a sample is novel is a classic problem within the broader field of pattern recognition~\cite{ruff2021unifying}. But merely detecting novelty is a limited task --- classification is far more useful mode of operation in machine learning. Most recognition work in computer vision has been conducted in a closed set classification mode, meaning all classes are known at both training and testing time. In contrast, OSR is a more realistic scenario, where partial  knowledge of the world is present during training, and unknown phenomena are guaranteed to appear during testing. The difficulty has been in finding effective approaches for distinguishing between known and unknown samples~\cite{geng2020recent}.

% SVM series
Scheirer et al. initially formalized the OSR problem~\cite{walter_open_set} and introduced the concept of~\textit{openness}, which characterizes the potential difficulty of open set problems. Importantly, they defined a notion of open space risk, based on the assumption that the farther away a sample is from the support of known training data in a feature space, the riskier it is to assign a known class label to it. Following this definition, a series of standalone classifiers was developed, including the 1-vs-Set Machine~\cite{walter_open_set}, $P_I$-SVM~\cite{pi-svm}, and Weibull-Calibrated SVM (W-SVM)~\cite{wsvm}. Moving beyond SVM-like classifers, Rudd et al. proposed the Extreme Value Machine (EVM)~\cite{Rudd_2018}, which is an OSR classifier based on the statistical Extreme Value Theory (EVT) that supports incremental learning.

% Deep network and so on series
OpenMax~\cite{Bendale_2016_CVPR} was the first OSR classifier that could be trained with a deep neural network, adapting EVT concepts to the activation patterns in the penultimate layer to perform OSR. Extending OpenMax, Generative OpenMax~\cite{g_openmax} trains a deep network with synthesized unknown data. Similarly, Counterfactual Images for
Open Set Recognition (OSRCI)~\cite{Neal_2018_ECCV} uses a Generative Adversarial Network (GAN) to generate unknown images that are close to the training images but technically do not belong to any training class.
Class Reconstruction Learning for Open Set Recognition (CROSR)~\cite{crosr} utilizes latent representations for reconstruction to improve performance on unknown samples.
The Class Conditioned Auto-Encoder for Open Set Recognition (C2AE)~\cite{c2ae} divides the training procedure into two sub-tasks, closed set classification and open set identification, and uses EVT to find a threshold for filtering unknown samples.
Class Anchor Clustering for Open Set Recognition (CAC-OSR)~\cite{cacosr} uses a distance-based loss function that forces known classes to form tight clusters around anchored class-dependent centers.
Multi-Task OSR~\cite{multi-task-osr} combines a classifier and a decoder network with a shared feature extractor network within a multi-task learning framework for OSR.

Outlier Exposure (OE) is another strategy for OSR, where outlier data is provided to the model during the training process so it can generalize and ideally detect unknown samples. It is possible to leverage outlier samples to improve anomaly detection by training anomaly detectors against an auxiliary dataset of outliers~\cite{Deep_Anomaly_Detection_with_Outlier_Exposure}. Dhamija et al.~\cite{Reducing_Network_Agnostophobia} introduced a new evaluation metric that focuses on comparing the performance of multiple approaches in scenarios where unknowns are presented and proposed novel losses that are designed to maximize entropy for unknown inputs. Kong and Ramanan~\cite{openGAN}  introduced OpenGAN, which augments training outliers with fake unknown data synthesized by a generator trained to fool the discriminator.

% Conclusion and connect next subsection
Considering all of the above approaches, the human capacity for managing novelty has been missing. The previous work has focused on formalizing the OSR problem and developing  methods that can improve OSR performance. However, none are informed by the measurement of human perception. This is surprising, considering that humans have a much stronger ability to perceive what belongs or doesn't belong to a task than computer algorithms. Different from previous OSR work, we suggest the use of visual psychophysics as a path forward. 

\textbf{Visual Psychophysics for Computer Vision.} Some researchers have attempted to draw a connection between the human visual system and artificial neural networks, looking into the differences between various visual systems~\cite{sensitivity}, as well as comparing the consistency between human vision and deep networks~\cite{DBLP:journals/corr/EberhardtCS16}.  Furthermore, a growing amount of work has been studying how human behavior and perception can be related to solving computer vision problems. For example, DiCarlo et al.~\cite{DICARLO2012415} highlighted how the human brain can perform object recognition despite a difficult environment and many variances in the setting. After reviewing the evidence from human behavior to neural recordings, they proposed that neuronal and psychophysical data is necessary for better computational models. Medathati et al.~\cite{MEDATHATI20161} presented an overview of computational approaches to biological vision, and showed how new computer vision methods can be developed from biological insights. And studies have found that the human visual system takes different amounts of time to respond to stimuli of varied difficulty~\cite{A_Computational_Perspective, Duncan1989VisualSA}.
All of these works touched on the notion that psychophysical methods show promise for computer vision algorithm development, but from the perspective of biology. 

From the perspective of computer vision, Scheirer et al. proposed the idea of \textit{Perceptual Annotation}~\cite{Scheirer_2014_TPAMI} to make use of psychophysical measurements collected via crowdsourced means to train more accurate SVM classifiers. McCurrie et al.~\cite{mccurrie2017predicting} collected behavioral data reflecting human judgments of subjective facial attributes in order to model them. Zhang et al.~\cite{zhang2018agil} suggested the
use of human gaze measurements, another  behavioral measurement type, for improving performance in  object-related tasks. RichardWebster et al.~\cite{brandon_psyphy,RichardWebster_2018_ECCV} proposed an evaluation framework for visual recognition models that constructs item-response curves made up of individual stimulus responses to find perceptual thresholds. %They later extended that work to highlight that psychophysical methods are viable for making automatic face recognition more explainable~\cite{RichardWebster_2018_ECCV}.

%Incorporating psychophysical data into the training process of a machine learning algorithm has been shown to be viable, but no work has been done on incorporating it into the novelty detection process. 
Most closely related to the work in this paper is that of Grieggs et al. \cite{grieggs2020measuring}, which introduces a psychophysical loss formulation for training artificial neural networks. In that work, behavioral experiments were conducted to collect reaction time data associated with the ability of reading in order to improve handwritten character recognition in historical documents. There are a few major differences between our work and~\cite{grieggs2020measuring}:
\textbf{(1)} We  develop a psychophysical loss function that incorporates several data streams and error measures.
\textbf{(2)} Our work focuses on the general area of image classification instead of the relatively niche area of historical document processing.
Not much expertise is required for our task, thus it is possible for us to conduct larger-scale human data collections.
\textbf{(3)} Our goal is to utilize the psychophysical loss to improve a deep network's performance on OSR, instead of just achieving better closed set classification performance. 

==> Arxiv submission file/sections/c_data.tex <==
\section{Psychophysical Study Of Known Data}
\label{sec:study}

To better understand how humans perceive familiar images in order to be tolerant to novelty, we designed and conducted a study using Amazon Mechanical Turk to collect human reaction time (RT) data\footnote{Approved by University of Notre Dame IRB under protocol 18-01-4341.}. As the source image data, we used a subset of ImageNet~\cite{ILSVRC15} that contains 335 classes (called ImageNet335 in this paper)~\cite{UMD_dataset}, which was created by the University of Maryland, Carnegie Melon University, and Columbia University as part of the DARPA Science of Artificial Intelligence and Learning for Open-world Novelty (SAIL-ON) program. For the purpose of novelty detection, we partitioned that dataset into two categories for machine learning. \textbf{(1)} \textit{Known Classes}: the classes with distinctly labeled positive training examples that appear at both training and testing time; these are the non-novel classes. \textbf{(2)} \textit{Unknown Classes}: the classes that are not labeled and are unseen in training; these are the novel classes used in testing.

With respect to the specific breakdown, we randomly selected 42 classes as unknown classes from ImageNet335, and the remaining 293 classes were used as known classes. In this study, we collected reaction time measurements for the detection of specific known samples in the midst of images from other classes. Knowing from previous work that a mix of original and psychophysically annotated training data tends to yield good results~\cite{Scheirer_2014_TPAMI, grieggs2020measuring}, we randomly chose 40 classes from the known classes to use in the human behavior experiments.

%\begin{table}
%\centering
%\resizebox{\columnwidth}
%{
%\begin{tabular}{| l | c | c |} 
%\hline
%\textbf{Category} & \textbf{Machine %Learning} & \textbf{Data Collection}\\ 
%\hline
%known known & 293 classes & 40 classes\\ 
%unknown unknown & 42 classes & 0 class\\
%\hline
%\end{tabular}
%}
%
%\vspace*{1mm}
% 
%\caption{Number of classes used for each category in ImageNet335 dataset for the machine learning study and human data collection, respectively. For the 293 known known classes, we treat them as their own class during model training and testing. And we randomly select 40 classes from those 293 classes and collected human reaction time on them. As for the 42 unknown unknown classes, we treat them all equally as one class during model testing, and we do not collect data on them.}
%\label{tab:all_data}
%\end{table}

% Table~\ref{tab:data_collection} shows the number of classes used for the human study. 
 %As for collecting data on novel samples, we used the images from all 78 known unknown classes from ImageNet413. We used images from known unknown classes for collecting data on non-novel samples because known unknown classes are used during the training and validation phases of the machine learning protocol, thus the corresponding reaction time entries can be used to train models with the proposed psychophysical loss. 
% \textcolor{blue}{A detailed list containing all of the classes for the data partitions and the classes chosen for the human study are included in this paper's Supplemental Material. (TBD)}

\textbf{Study Design.} While \emph{novelty} can be defined in different ways depending on the task and context, the problem we are trying to address in this research is class-level novelty. We designed a study that is suitable for collecting human reaction time measurements associated with known classes; we do this because unknown classes should not appear at training time in any capacity for a fair evaluation. Accordingly, we need a task that can provide information about the patterns of difficulty associated with known training samples as they interact with other classes. Here we can use other known class data as stand-in material for novel samples as RT measurements, which reflect difficulty, are made. 

\begin{figure}
    \centering
    \includegraphics[width=\columnwidth]{fig/survey_example.png}
    \caption{
        A sample of one of the survey questions for collecting human reaction time for known images.
        The subjects are asked to look at both rows of images and select the first image in the bottom row that is of the same object class as the reference class in the top row. It is possible that no image from the reference class is shown, hence the sixth option in the bottom row. In this specific example, the subjects should select the fifth image.
    }
    \label{fig:data_survey_design}
    \vspace{-5mm}
\end{figure}

%%% Cutting this to save some space. WJS
%At the beginning of the survey, the subjects are shown a page with an overview of the study. It provides critical information for the survey including a description, approval criteria, rejection criteria and methods for trouble shooting. After reading the introduction, subjects are led to a page that asks for their consent. It then proceeds to a direction page that helps subjects understand how they should answer the questions. As the last step before starting, the subjects are required to correctly answer a question as a practice. 

Each Mechanical Turk survey contained 25 questions, and subjects received 25 cents for completing a full survey.  Fig.~\ref{fig:data_survey_design} shows an example of one survey question (the full survey process is detailed in Supp.~Mat.~Sec.~1.1). In each question, two rows of images are shown to a subject. In the top row, five images are shown within a green box and are treated as reference images --- all of them from the same class. In the bottom row, five additional images are shown. The task is for the subject to look at the images in the bottom row sequentially from left to right in order to find the first image that belongs to the reference image class. If the subject believes that such an instance isn't present in the bottom row, then they can indicate that as their response. A timer is started when a question populates the page and is stopped when the subject makes a decision. This is the recorded reaction time that is associated with the image that belongs to the reference class in the question. If the correct answer is the sixth option (a quality control measure), then the subject's recorded answer and RT will not be used for machine learning training.

We consider the reference images in the first row of a question as training data for a human, and the images in the second row as testing data. Training images for our machine learning task are drawn from the correct known class images from the second rows across questions and surveys. The intuition behind this design is that RT on known samples provides more information on what is non-novel beyond a class label, and if a model has a better understanding of what is known, it should at the same time be able to better judge what could be unknown by increasing the separation between these two categories. This is consistent with a recent observation that novelty detection in deep networks works by detecting the absence of familiar features as opposed to the presence of novelty~\cite{dietterich2022familiarity}. Taking this idea a step further, the data from our study can be utilized effectively given a deep network with a notion of variable reaction time for each input~\cite{huang2018multiscale}, which is trained to enforce behavioral fidelity with humans.

% Similarly, when collecting reaction time on non-novel samples, a question has 5 reference images in the first row and 5 testing images in the second row. The difference is that among the 5 images but in the second row, 4 images are from a different class as the reference images, and 1 image is from the same class as the reference images. And the subjects are asked to find the image that shows a same type of object as the reference images. 

%After a subject finishes answering all the questions, they will receive a survey code at the end and they are required to submit the code to Mechanical Turk as the proof of their submission.

% Describe how we make the questions.
We pick one known class for the first row training data and another known class as a stand-in novel class that is different from the training data for the second row testing data. To be specific, in a question whose answer is not the sixth option, there are 5 images that are from a single class in the first row; in the second row, there are 4 images that are from a different class and 1 image that is from the same class as the first row. Such a design is straightforward for subjects to understand because there are only 2 classes shown at a time in a question, thus we expect to minimize noise in the results.
Assuming we pick $n$ classes for the surveys, each class is paired with itself and the rest of the $n-1$ classes. Using each pair, 20 questions are created, and based on the above there are $n^2$ different sets of surveys for the $n$ classes chosen. In the experiments conducted there are 40 known classes, thus there are 1,600 sets of different surveys in total.

To filter out bad submissions, we also include five control questions in every survey, which means each survey has 25 questions in total. These control questions are designed to be trivially easy so that any diligent worker will most likely get them correct. We allow the subjects to answer at most two control questions incorrectly. Answers provided by unreliable subjects are filtered out and are not considered for the machine learning experiments. Subject were not able to answer the same question twice. 
 Valid response times had to be under 28 seconds (the maximum RT after removing the largest RT values reflecting 5\% of the total data) on the assumption that anything longer reflected an inattentive subject. Although we instructed the subjects to look at the images from left to right sequentially, there was no control to enforce this on their side. Thus we require that 5 subjects complete each question so that noise can be smoothed out by considering average reaction times for each image. To ensure the order of the images does not affect the reaction time entries, all the images are selected randomly when the survey is generated and the images do not follow any pre-set order.

%%% Too much detail. WJS
%after subjects have submitted their answers, we check the survey code they provide. When subjects answer more than 2 control questions incorrectly, their survey codes start with a certain pattern that we can recognize, and we discard all the answers submitted by these users.

%%% Too much detail. WJS
%In addition, we also remove outlier responses. When processing the data, we noticed that the maximum reaction time among all entries was over 1000 seconds. When plotted, the distribution of recorded reaction times has a very long tail, which indicates that not all the entries should be used. We anticipated that some subjects may end the survey without finishing it, or leave the page as-is while doing other things, or there could simply be a server error; these situations are out of our control and can lead to extremely long reaction times that should not be used in our machine learning experiments. We plot multiple figures by manually picking different thresholds on reaction time, and come to a conclusion that we remove 5\% of the longest reaction times as the outliers (shows as in Figure \ref{fig:rt_dist}), which makes the maximum reaction time to 20 seconds for the whole dataset.

\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{fig/rt_known_density_kernellabel4.pdf}
    \caption{
        This histogram and kernel density estimate shows the distribution of human reaction time for the data collected for known samples.
        The X-axis shows the range of reaction times after thresholding the long tail, which removed outliers. The Y-axis shows the probability of occurrence.
        }
    \label{fig:rt_dist}
    \vspace{-5mm}
\end{figure}


% idk paragraph point
\textbf{Summary of Collected Data.} We collected 211,074 RT measurements in total. After data cleaning and data pre-processing, we sampled 121,073 instance-level RTs for model training. We grouped the RTs that belong to the same image and calculated the average of them, and we used this average value to represent the RT for an image. Overall, there are 33,548 training samples from the 40 known classes, and 12,428 images among them have corresponding RTs.

After collecting the RT data, an important question for the subsequent machine learning work was whether to use class-level or sample-level behavioral information in the loss formulation. We started by looking at class-level RT by generating box plots summarizing the measurements by class pairings for each class (see Supp.~Mat.~Sec.~1.2). To be useful for a loss function, large relative differences between a class and its different pairings would need to be present. We observed that the variance in RT within a class across its various other-class pairings was small, and that the various pairings have similar minimum and median RT statistics. This indicates that there isn't enough RT information at the class-level to be useful for a loss function, as patterns of difficulty across different classes cannot be ascertained.

Next, we turned to the sample-level behavioral information. We plotted the distribution of RT measurements for these known samples, shown in Fig.~\ref{fig:rt_dist}.
Looking at the distribution, there is a large amount of variance across samples from all of the classes. This means that some samples have longer RT measurements while others have shorter ones, regardless of the classes they come from. Therefore the understanding and usage of RT has to be taken down to the sample-level for the design of the loss function.
Our RT data indicate that the human visual system is perceiving each sample differently. Using this finding as an intuition for machine learning, we make the following assumption: human RT is a significant indicator of the latent difficulty of perceiving an object relative to objects from other classes,  meaning these measurements will be useful or supervised training because the training set captures those relative comparisons.

==> Arxiv submission file/sections/d_approach.tex <==
\section{Training a Model with Variable Reaction Time}
\label{sec:approach}

With a large number of reaction time measurements associated with individual training points, we need some efficient way to make use of that data for training a deep network. The most straightforward approach has been to incorporate such data into a loss function~\cite{Scheirer_2014_TPAMI, grieggs2020measuring}.
Unexplored before in the OSR literature, however, is a tighter coupling between human and model behavior when it comes to the reaction time associated with inputs.
Thus we propose to enforce human behavioral fidelity in a model that supports dynamic reaction time during runtime (Fig.~\ref{fig:pipeline}). This is accomplished via a new psychophysical loss function that encourages the model to mimic per instance human RT.

%To match human reaction time and model reaction time, thus enforcing proportional behavior between human perception and model training, we need to ensure that the structure of the network adequately reflects the variance in machine reaction time.

\begin{figure}
    \centering
    \includegraphics[width=\columnwidth]{fig/psychophysics_pipeline_inference.png}
    \caption{
        Pipeline depicting the three components of the proposed machine learning process.
        The yellow box represents the human study for collecting RT. %, where we pick 40 known classes and use them for the survey on Amazon Mechanical Turk to obtain instance level human RT.
        The blue box shows machine learning training. % During training, training and validation data is sent into MSD-Net; the human RT is used at the same time to train the network with the proposed psychophysical loss function.
        %During training, we obtain probabilities from validation data every few epochs and update the training thresholds with them. After training is done, we obtain inference threshold by running validation data through the best model.
        The green box illustrates the testing process. See Supp.~Mat.~Sec.~3.1 for additional detail on these.
        %We send testing data into a trained MSD-Net model and get exit indices and probabilities for all of the exits, checking the probability for each exit.
       % When a certain exit's max probability is larger than the threshold from validation data and the model is making a correct prediction, we consider it a correct result for the purpose of evaluation metric calculation. 
    }
    \label{fig:pipeline}
    \vspace{-5mm}
\end{figure}

\textbf{Multi-Scale DenseNet.}
Most network architectures use approximately the same amount of time to process all input images. Typically, networks only have one classifier at the end of the architecture, and it is extremely difficult, if not impossible, to discern any meaningful difference in model reaction time between samples.
To be able to support different model reaction times and to train the model with human RT data, we chose to use the Multi-Scale DenseNet (MSD-Net)~\cite{huang2018multiscale} architecture with a custom loss function. We also describe an experiment for a variant of ResNet-18 in Supp.~Mat.~Sec.~3.2.

Different from many other networks that only have one classifier at the end, MSD-Net has five classifiers in its architecture.
Utilizing these classifiers as model exits, we modify the network to output the predictions after each classifier, and use a thresholding strategy to determine whether the network is confident enough to decide which class a sample should be classified into, or whether a sample is unknown. 
We start training by setting all 5 thresholds corresponding to each exit to zero. To update these thresholds, we extract the prediction scores on validation data every 5 epochs at each exit, taking the median of all the prediction scores for a specific exit as its threshold. These updates are necessary because the model behavior changes over time, and probabilities become higher as the model better describes the data. 

We call these thresholds \emph{training thresholds}.
If the network produces a prediction score that is above the threshold and outputs a correct prediction, a sample is considered to be exiting the network. We consider it important that a sample has to satisfy both conditions during training because we need to enforce the constraint that the network confidently makes correct predictions. Training thresholds are updated based on the probability vectors from the exit loss  described below.

\textbf{Psychophysical Loss Formulation.}
The base loss used for training MSD-Net is the common multi-class classification cross-entropy loss.
The cross-entropy loss is the function
\begin{equation}
    \Loss_C(p, q) = -\sum_{y\in Y} p(y) \log q(y)
\end{equation}
 where $p$ is the labeled probability (one-hot vector) of the class $y$ from the closed set of classes $Y$ and $q$ is the MSD-Net predicted probability of the class $y$.
Here we add to the cross-entropy loss by incorporating RT measurements via two additional psychophysical loss functions.
This is accomplished via a weighted summation of the cross-entropy loss and a psychophysical loss.

% The first psychophysical loss is the performance loss:
% \begin{equation}
%     \Loss_{P}(x) = \frac{R_\text{max}-R_\text{x}}{R_\text{max}}
% \end{equation}
% where $R_{max}$ is the maximum human RT across all of the human training data and $R_{x}$ is the mean human RT of the current image $x$.
% $\Loss_{P}$ is then the image's reaction time score normalized by $R_{max}$ to be within the range $[0, 1]$.
% Based on the dataset described in Sec.~\ref{sec:study},
% $R_{max}$ was found to be 28 seconds.
% This loss is the psychophysical loss proposed in \cite{grieggs2020measuring} when it is combined with cross-entropy loss in a weighted summation.
% The performance loss leverages the information of the expected human reaction time versus the maximum RT to inform the model of the sample's difficulty for human classification.
% This relies on the assumptions that human RT is longer for images that are more difficult to classify by the humans and that this difficulty should be shared between humans and the model. 
% %should capture information from the humans about the sample to better inform the model.
% The performance loss forces the MSD-Net to weight the samples humans quickly classified so that they have more impact on the loss, encouraging the network to learn these samples more quickly than those that are more difficult for humans to process.

The psychophysical loss is an exit loss
\begin{equation}
    \label{eq:three}
    \Loss_{E}(x, \hat{y}) = \left| {\Exit_{\mathrm{target}(x)}} - \Exit_{\hat{y}} \right| 
\end{equation}
where $\Exit_{\hat{y}}$ is the exit integer index of the MSD-Net prediction $\hat{y}$, and $\Exit_{\mathrm{target}(x)}$ is a lookup function that returns the target exit index for the sample $x$.
The exit loss is designed to push the MSD-Net's reaction time for the sample to be proportional to the sample's target exit based on a binning strategy informed by the human RT measurements.
% Both $\Exit_\text{target(x)}$ and $\Exit_{\hat{y}}$ are integers, and ranged from 

%% TODO: Review and Clean:
To obtain the exit loss, the following two factors must be measured. \textbf{(1)} Expected exit: $\Exit_{\mathrm{target}(x)}$.
    This value is assigned by measuring a discrete distribution of human reaction time.
    After removing the outliers from the human RT measurements and obtaining the minimum and maximum values, the entire range is discretized into five bins %to smaller ranges
    in accordance with the number of classifiers in the MSD-Net architecture.
    The cut-off thresholds defining the ranges covered by each bin are the quintiles of human RT in Fig.~\ref{fig:rt_dist} and are shown in Supp. Table 2.
    When a sample enters the network for training, the human RT associated with that sample is checked, and the corresponding exit index from the upper bound of the range is used as its $\Exit_{\mathrm{target}(x)}$.
    For instance, if a known sample has an average human RT of 5.5 seconds, its $\Exit_{\mathrm{target}(x)}$ will be 2.
    \textbf{(2)} Predicted exit for a sample determined by when it leaves the network: $\Exit_{\hat{y}}$.
    As a sample is processed through each classifier, the model checks the prediction scores as well as predicted label for that classifier.
    If the maximum prediction score produced is larger than the set threshold for an exit and the prediction is correct, the sample is considered to be leaving the network and the index of the exit is $\Exit_{\hat{y}}$.

The complete proposed psychophysical loss combines the  cross entropy loss and the exit loss as a weighted summation:
%\begin{multline}
\begin{equation}
\begin{aligned}
    \Loss_{\Omega}(p, q, x, \hat{y}, \vec{\omega}) = &
        ~\omega_C \Loss_C(p, q) \\
        & +  \omega_E \Loss_{E}(x, \hat{y})
    \label{eq:loss}
\end{aligned}
\end{equation}
%\end{multline}
where $\vec{\omega} = [\omega_C, \omega_E] : \omega_i \in \mathbb{R}$ is a vector of weights that correspond to the hyperparameter weighting of each component.
%We optimize the exit loss by minimizing the L-1 distance between target exit and predicted exit, thus matching model behavior with human perception.

% \begin{table}
% \setlength{\tabcolsep}{1.0\tabcolsep}
% \centering
%  \begin{tabular}{| c | c | c | c | c | c |} 
%  \hline
%   & $20\%$ & $40\%$ & $60\%$ & $80\%$ & Max\\ 
%  \hline
%  Reaction Time & 3.5720 & 4.9740 & 7.0156 & 11.601 & 27.572 \\
%  \hline
% Exit Index & 0 & 1 & 2 & 3 & 4  \\
%  \hline
%  \end{tabular}
%  \vspace*{1mm}
%  \caption{The cut-off thresholds for human reaction time for known known samples. Minimum (Min) is set to 0, and other 5 thresholds are obtained by percentile, all the values for Reaction Time are in seconds.}
% \label{tab:rt_dist}
% \end{table}

\textbf{Training and Validation Pipeline.} We take an original training dataset of images that do not have associated RTs and split it into training and validation sets with a ratio of 70\% for training and 30\% for validation. Available samples that do have associated measured RT are proportionally split via the same ratio into training and validation sets and merged with the samples that do not have any associated RT. We utilize an existing implementation of MSD-Net (\url{https://github.com/kalviny/MSDNet-PyTorch}), and send training and validation data into the network to train it with the psychophysical loss. 
%With respect to threshold updates during training, prediction scores are obtained from the validation set every 5 epochs, with the median of the probabilities calculated for each exit respectively. These medians are then used as the updated thresholds. Thresholds are updated until the full training process is complete. 
Optionally, the weights in $\vec{\omega}$ can be set via domain knowledge or hyperparameter optimization. In our experiments, all the weights were set to 1.0 to assess base performance.

\textbf{Testing Pipeline.} After obtaining a model from training, we perform post-processing for novelty detection. First, we need to determine the threshold for each exit. This leads to a different set of thresholds than the training thresholds; we call these \textit{inference thresholds}. To obtain this set of thresholds, the \textit{best model} needs to be identified first. During the training phase, we save a model as well as the training and validation accuracy associated with it at every epoch. After training is done, the model that produced the highest top-1 validation accuracy is selected as the best model. We then run validation data through this best model and calculate the median of all the predicted scores for each exit respectively; these median scores are considered to be the inference thresholds. They remain static from this point forward because the best model is finalized. We then run all test samples from both known and unknown classes through the selected model, saving the prediction scores from each exit. Lastly, the inference thresholds are applied to these scores to find out when the samples leave, with corresponding exit indices  recorded. % well as calculating all the evaluation metrics. 

The exit strategies are slightly different for known samples and unknown samples. For all the known samples, a sample correctly exits the network when the maximum score is larger than a given inference threshold, and when the network makes a correct prediction. If a sample does not exit from one of the first 4 exits due to being under threshold each time, it comes to the final exit, where there are three possibilities for it.
\textbf{(K1)} The maximum score of a sample is larger than the given threshold, and the prediction is correct: the sample exits and is correctly classified as a known class. \textbf{(K2)} The maximum score of a sample is larger than the given threshold, but the prediction is wrong: the sample exits and is classified as known, but associated with an incorrect class. \textbf{(K3)} The maximum score of a sample is smaller than the given threshold: the sample exits and is classified as unknown, making it a false negative.

As for testing unknown samples, there are only 2 possible cases for each sample. \textbf{(U1)} The maximum score is smaller than the given threshold at every exit: the sample is classified correctly as unknown. \textbf{(U2)} The maximum score at a particular exit is larger than the threshold given by that exit: the sample is wrongly classified as known, which makes it a false positive.

For testing known and unknown samples, we use the probability scores produced by the SoftMax function, and the exits solely decide whether a sample is known or unknown. During the testing phase, all samples are processed through the 5 exits and the probability scores from each exit are saved. The  scores are then post-processed to obtain the final classification results.

%%% Too much repeated text here. I integrated the new bits above. -WJS.

%\textbf{Different Thresholds for Training and Testing.} %\textcolor{red}{We emphasize that we use 2 different set thresholds for training and testing, respectively.} 

%\textcolor{red}{The training threshold is applied to %training phase only. As mentioned earlier in this %section, training threshold is updated every 5 epochs %by calculating the median of validation probabilities %at each exit, till training is done. Updating training %threshold is necessary because the model behavior %changes constantly, and probabilities become higher as %the model describe the data better.}
%
%\textcolor{red}{After training is done, we are able to select one model that has the highest top-1 validation accuracy as our best model, and we ran validation data through this model to obtain our inference threshold. Our inference threshold stays static because the best model is finalized and does not change anymore.}

==> Arxiv submission file/sections/e_result.tex <==
\section{Experiments and Results}

%In this section, we provide details on our experimental results for OSR. Importantly, we highlight the improvement obtained by training MSD-Net with the proposed psychophysical loss. We also run experiments for a large selection of other OSR methods for comparison. The provided analysis of the results is intended to surface insights for the significance of human perception in deep model training for OSR settings.

% \textbf{Experiments: Processing Pipeline.} As shown in Fig.~\ref{fig:pipeline}, our pipeline consists of three major components: human experiments for data annotation, the MSD-Net training pipeline, and the post-process evaluation pipeline. 

% \textit{Human Annotations.} As described in Sec.~\ref{sec:study}, we distribute surveys on Amazon Mechanical Turk to gather human RT for training data. During the data collection process, we obtain 5 reaction times for each sample to be more accurate statistically. After filtering out outliers, we take the average of all the reaction times associated with a sample that are left and use that mean value as the sample's corresponding RT for training.
% \textit{Training and Validation Pipeline.} We take an original training dataset of images and split it into training and validation sets with a ratio of 70\% for training and 30\% for validation. Other available samples that have associated measured RT are proportionally split into training and validation sets, and merged with the samples that do not have any associated RT. We utilize an existing implementation of MSD-Net (\url{https://https://github.com/kalviny/MSDNet-PyTorch}), and send training and validation data into the network to train it with the psychophysical loss. As mentioned in Sec.~\ref{sec:approach}, we need a threshold for each exit to decide when a sample exits. When training starts, the thresholds for the 5 exits are all set to zero by default. After that, probabilities are obtained from the validation set every 5 epochs, with the median of the probabilities calculated for each exit respectively, which are then used as the updated thresholds. We keep updating the thresholds till the full training process is done.

% \textit{Testing Pipeline.} After obtaining a model from training, we perform post-processing for novelty detection. First, we need to determine the threshold for each exit, this is a different set of thresholds than the ``training thresholds" we describe in Sec.~\ref{sec:approach}, and we call it ``inference thresholds". We obtain this set of thresholds by running validation data through the \textit{best model}, which is the model that produces the highest top-1 validation accuracy, by calculating the median of all the predicted scores (probabilities) for each exit respectively, and using those median scores as exit thresholds. We then run all test samples from both known known and unknown unknown classes through the selected model and we save the probability scores from each exit. Lastly, we apply the thresholds to these probabilities to find out when a sample leaves, and at the same time we record the corresponding exit index. % well as calculating all the evaluation metrics. 

% It is worth mentioning that the exit strategies are slightly different for known samples and unknown samples. For all the known samples, a sample correctly exits the network when the maximum probability is larger than a given threshold, and when the network makes a correct prediction. If a sample does not exit from one of the first 4 exits due to being under threshold each time, it comes to the final exit, where there are three possibilities for it.
% \textbf{(K1)} The maximum probability of a sample is larger than the given threshold, and the prediction is correct: the sample exits and is correctly classified as a known class. \textbf{(K2)} The maximum probability of a sample is larger than the given threshold, but the prediction is wrong: the sample exits and is classified as known, but associated with an incorrect class. \textbf{(K3)} The maximum probability of a sample is smaller than the given threshold: the sample exits and is classified as unknown, which makes it a false negative.

% As for testing unknown samples, there are only 2 possible cases for each sample. \textbf{(U1)} The maximum probability is smaller than the given threshold to that exit at every exit: the sample is classified correctly as unknown. \textbf{(U2)} The maximum probability at a particular exit is larger than the threshold given by that exit: the sample is wrongly classified as known, which makes it a false positive.

\textbf{Data and Evaluation Metrics.}
 %As mentioned in Sec.~\ref{sec:study}, we use a subset of ImageNet designed for OSR in our experiments.  For training, 293 classes with a total of 33,548 images were chosen --- all of them are considered known classes. Among these 293 classes, 12,428 images from 40 classes have associated human RT measurements. 
The training data breakdown can be found in Sec.~\ref{sec:study}.
For validation, 9,058 images are available from the 293 known classes. %Some 3,778 images have reaction times with them; these are drawn from the same 40 classes with associated RT in the training set. 
The test set consists of known and unknown images. The known test partition consists of the 293 classes seen in training providing a total of 336,453 new images.
The unknown test partition consists of 42 classes unseen at training --- all are considered to be part of one unknown class with 48,067 images. 

Although various OSR works~\cite{Neal_2018_ECCV, crosr, cacosr} use AUROC as a metric to evaluate  performance, we believe that it is somewhat flawed for this problem. 
Importantly, it obscures the performance achieved through the use of a single threshold by combining a large range of thresholds to produce one score. Moreover, it does not provide a recommendation for selecting the best threshold. AUROC can be used fairly as a metric to assess a model's performance during training or validation, but there should only be one threshold per classifier used in the testing phase, as would be done in operation. Knowing this, we chose to use fixed thresholds obtained via experiments with the validation data as our inference thresholds.

%\textcolor{red}{(Need to elaborate why AUROC alone is not a good metric)}. 
%Besides, we do not change the threshold for Open-Set Recognition and we are using thresholds obtained from validation data. 
 
As OSR is a task built on top of novelty detection by adding multi-class classification for known samples, both the detection and classification components can and should be evaluated separately. Thus we include metrics for both when reporting our results. 
%For novelty detection, we include True Positive (TP), True Negative (TN), False Positive (FP), False Negative (FN), F1 Score and the Matthews Correlation Coefficient (MCC). For classification, we use accuracy score and consider top-1 accuracy for testing known samples and accuracy for testing unknown samples.
For novelty detection, we consider accuracy when testing unknown samples. For multi-class classification, we use accuracy score and consider top-$n$ accuracy for testing known samples. We report counts for True Positives (TP), True Negatives (TN), False Positives (FP), and False Negatives (FN), as well as F1 Score and the Matthews Correlation Coefficient (MCC) in the Supp.~Mat.~Sec.~3 for comparison.

\textbf{Results: Contribution of Each Loss Function.}
Since the proposed psychophysical loss is composed of an exit loss added on top of a cross-entropy loss, we trained two models separately: one model is trained just with cross-entropy loss and the other is trained according to Eq.~\ref{eq:loss} (the proposed loss). To compare the performance of our loss formulation with the previous published psychophysics loss \cite{grieggs2020measuring}, we also trained a model with this \textbf{performance loss}. It is noted as $\Loss_P$, and is added on top of cross-entropy loss as another baseline.

We train each of the models using a single GPU with a batch size of 16 images shaped 224x224 and an initial learning rate of 0.1 for 200 epochs. As for the optimizer, we use stochastic gradient descent (SGD) with a momentum of 0.9 and a weight decay of 0.0001. All other parameters are set the same as the original implementation, and we did not heavily tune these training parameters. Evaluation takes place in a 5-fold manner, training models with 5 different fixed seeds in all cases. The average accuracy over all folds is considered as the final result. 

%During the training and validation phases, one model and the training and validation accuracy associated with it is saved to disk after each epoch, which means we have 200 models for a loss function and a seed when training is done. We find the model among all 200 that has the highest top-1 validation accuracy, and use it as the \textit{best model} for our testing process. We recognize that the performance reported may not be reliable if we train models with randomly generated seeds, and we need to avoid cherry picking on seeds. To address this and to be specific, we train models with each loss with 5 manually selected seeds 0, 1, 2, 3 and 4 for 200 epochs each, and find the \textit{best model} for each seed respectively, and we calculate the average performance from all 5 seeds for our final results.


\begin{table}
\centering
\resizebox{\columnwidth}{!}{
\begin{tabular*}{\columnwidth}{@{\extracolsep{\fill}}|c|c|c|c|c|}
\hline
 %\textbf{Category} & $\bm{Loss_C}$ & $\bm{Loss_C + Loss_P}$ & \textbf{Prop. (Eq.~\ref{eq:loss})} \\
 %\textbf{Category} & $\bm{\Loss_C}$ & $\bm{\Loss_C + \Loss_P}$ & $\Loss_\Omega$ \textbf{(Eq.~\ref{eq:loss})} \\
 %\textbf{Split} & \textbf{Accuracy} & $\Loss_C$ & $\Loss_C + \Loss_P$ & $\Loss_C + \Loss_P + \Loss_E$ \\
 \textbf{Split} & \textbf{Accuracy} & $\Loss_C$ & $\Loss_C + \Loss_P$ & $\Loss_C + \Loss_E$ \\
\hline
  train & known top-1 & \textbf{72.56}$\pm0.47$ & \textbf{72.56} $\pm~0.27$ & 72.10$\pm0.42$ \\
  train & known top-3 & 85.01$\pm0.28$ & \textbf{85.09} $\pm~0.20$ & 84.35$\pm0.27$ \\
  train & known top-5 & 89.02$\pm0.22$ & \textbf{89.19} $\pm~0.15$ & 88.37$\pm0.22$ \\
\hline
  valid. & known top-1 & 53.98$\pm0.30$ & 52.90 $\pm~0.51$ & \textbf{60.00}$\pm0.27$ \\
  valid. & known top-3 & 68.76$\pm0.32$ & 68.36 $\pm~0.20$ & \textbf{72.12}$\pm0.28$ \\
  valid. & known top-5 & 74.67$\pm0.38$ & 74.18 $\pm~0.13$ & \textbf{77.34}$\pm0.18$ \\
\hline
  test & known  top-1 & 26.67$\pm7.76$ & 28.68 $\pm~6.91$ & \textbf{36.48}$\pm0.43$ \\
  test & known  top-3 & 36.40$\pm10.99$ & 38.90 $\pm~9.87$ & \textbf{46.70}$\pm0.73$ \\
  test & known  top-5 & 41.08$\pm12.24$ & 43.76 $\pm~11.14$ & \textbf{51.00}$\pm0.89$ \\
  test & unk. top-1 & 21.05$\pm0.63$ & 23.95 $\pm~2.98$ & \textbf{54.23}$\pm0.48$ \\
\hline
\end{tabular*}}
    
    \vspace*{1mm}
    \caption{
        Results for three variations of the loss used to train MSD-Net; scores are accuracy (\%).
        For each loss, we run experiments 5 times using 5 different seeds for training; the scores shown for each experiment are the average of 5 runs with standard error. $\Loss_P$ is a performance loss~\cite{grieggs2020measuring} described in Sec.~2 of the Supp.~Mat. 
        Additional results, including results for a model trained with all 3 losses and complete results for all 5 runs, are in Sec.~3 of the Supp.~Mat.
    }
\label{tab:three_baselines}
\vspace{-8mm}
\end{table}


Table~\ref{tab:three_baselines} shows the training, validation and testing results for this experiment.
All three configurations of the loss demonstrate roughly the same accuracy on known samples during training. When performance loss is added to cross-entropy loss, there is a noticeable uptick in test accuracy for both known and unknown samples. This indicates that measured RT is helping the trained model to generalize in the OSR setting. The increased performance in this case on known samples is consistent with prior work~\cite{grieggs2020measuring}, but the increase in performance on unknown samples is a new finding. Better conditioning of the MSD-Net exit behavior yields even more performance improvement. 
For top-1 validation accuracy, the proposed loss %$\Loss_\Omega$
of Eq.~\ref{eq:loss} outperforms the cross-entropy loss by 6.02\%, and the combined cross-entropy and performance loss by 7.1\%. Even more significant improvement is demonstrated in the testing phase.
When testing on known classes, the proposed loss results in a top-1 accuracy of 36.48\%,  outperforming the two other loss configurations (26.67\% and 28.68\%). When detecting unknown samples, the proposed loss largely outperforms the others with 54.23\% accuracy, compared to 21.05\% and 23.95\%. These results show that our proposed loss leads to models that are able to maintain good performance when testing with multiple known classes while simultaneously rejecting unknown samples.

\textbf{Results: Other Baselines.}
We also compared our method with eight other OSR methods from the literature. With respect to standalone classifiers, we evaluated SVM~\cite{svm} with thresholding, $P_I$-SVM~\cite{pi-svm}, W-SVM~\cite{wsvm}, and the EVM~\cite{Rudd_2018} with  MSD-Net features. With respect to deep learning-based methods, we evaluated OpenMax~\cite{Bendale_2016_CVPR}, OSRCI~\cite{Neal_2018_ECCV}, CROSR~\cite{crosr}, and CAC-OSR~\cite{cacosr}. See Supp.~Mat.~Sec.~2 for descriptions of these approaches. For these experiments, we used the same dataset used to evaluate MSD-Net training with different loss configurations. As we did not heavily tune hyperparameters in our proposed approach to avoid overfitting, for a fair comparison we also refrained from doing so for all baseline methods. 
Table~\ref{tab:all_results} shows results on known samples and unknown samples from the test set for all methods, including the different configurations of MSD-Net training. 

%%%%%

%\subsubsection{Metrics}
%We use multiple metrics to comprehensively evaluate these methods, and we also include the two baselines described in section 5.3.

%\textcolor{red}{Need to say why F-1 is not a good metric/not enough to evaluate the performance of a model?? Also do we need to explain each metric, or can we just assume the readers should know what they are...?}

%\textcolor{red}{mention all the weights are just one}

While most of the methods only achieve performance that is only a little better than making a random choice among the 293 known classes, the different configurations of MSD-Net training achieve excellent top-1 accuracy when testing on known samples, with the proposed loss yielding the best result.
The EVM has the highest accuracy when tested with unknown samples, but when we look at the accuracy for known samples, we notice that it tends to classify everything as unknown.
Similar to the EVM, CROSR and CAC-OSR also classify most of the samples as unknown, leading to a high accuracy when considering just the unknowns, but very poor accuracy for known samples.
Reversing this trend, OSRCI classifies most of the classes as known, which indicates it produces high prediction scores for both known and unknown samples, but is not able to distinguish between known and unknown samples, and at the same time classifying known samples into wrong classes. SVM and OpenMax are more balanced when it comes to OSR and are reasonably accurate in detecting unknown samples, but like other algorithms, they failed to perform well when assigning known samples to the correct class. Only the MSD-Net configurations are able to maintain good performance for both novelty detection and classification. 

\begin{table}[t]
  \centering
  \begin{tabular*}{\columnwidth}{@{\extracolsep{\fill}}|c|c|c|}
  \hline
    \textbf{Algorithm} & 
    \textbf{Test Unknown Acc.} & 
    \textbf{\begin{tabular}{@{}c@{}} Test Known \\ Top-1 Acc\end{tabular}} \\
    \hline
    SVM~\cite{svm} & 55.04\% $\pm~0.76$ & 0.60\% $\pm~0.07$ \\
    \hline
    $P_I$-SVM~\cite{pi-svm} & 8.31\% $\pm$ 0.12 & 0.28\% $\pm$ 0.02 \\
    \hline
    W-SVM~\cite{wsvm} & 9.21\% $\pm$ 0.15 & 0.09\% $\pm$ 0.01 \\
    \hline
    EVM~\cite{Rudd_2018} & \textbf{{\color{red}{99.39}\%}} $\pm$ 0.00  & 0.45\% $\pm$ 0.00 \\
    \hline
    OpenMax~\cite{Bendale_2016_CVPR} & 32.41\% $\pm$ 0.04 & 0.39\% $\pm$ 0.00\\
    \hline
    OSRCI~\cite{Neal_2018_ECCV} & 1.11\% $\pm$ 0.01 & 0.36\% $\pm$ 0.00 \\
    \hline
    CROSR~\cite{crosr} & 85.78\% $\pm$ 0.00 & 1.92\% $\pm$ 0.00 \\
    \hline
    CAC-OSR~\cite{cacosr} & 94.55\% $\pm$ 0.00 & 0.05\% $\pm$ 0.00 \\
    \hline
    MSD-Net $\Loss_C$ & 21.05\% $\pm$ 0.63 & 26.67\% $\pm$7.76 \\
    \hline
    MSD-Net $\Loss_C + \Loss_P$~\cite{grieggs2020measuring} & 23.95\% $\pm$ 2.98 & 28.68\% $\pm$ 6.91 \\
    \hline
    MSD-Net $\Loss_C + \Loss_E$ (Eq.~\ref{eq:loss}) & 54.23\% $\pm$ 0.48 & \textbf{36.48\%} $\pm$ 0.43 \\
    \hline

  \end{tabular*}
  
  \vspace*{1mm}
  \caption{Testing results for the proposed loss and other baselines. Bold numbers indicate best performance for a metric. Results in red highlight spurious best results due to a classifier biased towards determining samples are novel. }
  \label{tab:all_results}
  \vspace{-8mm}
\end{table}

The poor performance of the baseline approaches on the ImageNet335 OSR task was surprising. The most significant cause is likely dataset size. As emphasized earlier, OSR research tends to use a handful of small datasets with far fewer than 335 classes. Testing performance is known to drop when the number of classes increases~\cite{geng2020recent}. Further, we have intentionally curated the dataset used in this paper to provide relatively few examples per class in order to assess the impact of adding behavioral data. Larger-scale OSR work has made use of Tiny ImageNet~\cite{Neal_2018_ECCV, crosr,cacosr} or full ImageNet pre-training~\cite{Bendale_2016_CVPR,Rudd_2018} with access to hundreds of thousands of labeled images for training --- an order of magnitude more data than what is available in our experiments for training. Our proposed approach gains information from the behavioral data that partially compensates for having fewer training samples per class, which otherwise heavily degrades performance. 

Secondary reasons for poor performance include input image size sensitivity for deep learning-based models and feature size constraints for standalone classifiers. In the former case, to be able to use this data with the baselines, we had to downscale the images to match the input size required by each baseline method, which potentially led to a loss of information when they were trained. In the latter case, we had to use PCA to reduce the dimensionality of the MSD-Net features for a few of the baseline methods (details can be found in Supp.~Mat.~Sec.~2), including: SVM, W-SVM, $P_I$-SVM and EVM. Such brittleness needs further attention in OSR work. 

% \textit{Others} \textcolor{red}{(We found out that there is a flaw in the design of OpenMax. OpenMax uses the features that are predicted correctly to calculate MAV, distances and so on, but it is possible that no sample in a class is predicted correctly, if a dataset is complex/difficult.)}


==> Arxiv submission file/sections/f_discussion.tex <==
\section{Discussion}

Table \ref{tab:all_results} shows testing results on known samples and unknown samples for all methods including model trained with our psychophysical loss, and the bold number in each column indicates the method that has the best performance on that metric.

While most of the methods only achieve a performance that is only a little better than making a random choice among 293 known class, Cross-Entropy, Cross-Entropy with performance loss and psyphy model maintain excellent top-1 accuracy on testing on known samples. EVM has the highest accuracy when tested with unknown samples, but when we look at other metrics all together, we notice that it tends to classify everything as unknown. Similar with EVM, CROSR and CAC-OSR also classify most of the samples as unknown, leading to a high accuracy on testing unknown, but a high number of false positive. On the other hand, OSRCI classifies most of the classes as known, which indicates it produces high probability scores for both known and unknown samples, and it is not able to distinguish known and unknown. SVM and OpenMax are more balanced when it comes to Open-Set Recognition and produce decent accuracy score while tested with unknown samples, and they also both generate good F-1 scores; but like other algorithms, they failed to perform well on the closed-set part to classify known samples into a correct class. Only the last 3 methods shown in the table are able to maintain good performance on testing known samples, and distinguish unknown from known at the same time; and overall, our psyphy model achieves highest performance on testing top-1 accuracy, F1-score and MCC.

We look more closely into each method and the result we have to analyze the reasons why some methods failed on the task.

\textcolor{red}{I feel we should mention why we used fixed threshold? Where to put it}

\begin{itemize}
    \item \textbf{Dataset Size: } Most of the Open-Set Recognition papers utilize a few standard datasets, including but not limited to LETTER (26 classes), PENDIGITS (10 classes), COIL20 (20 classes), MNIST (10 classes), SVHN (10 classes), CIFAR-10 (10 classes), CIFAR-50 (50 classes) \textcolor{red}{(need to double check this one)} and Tiny-ImageNet (200) classes. Most of these datasets do not contain a large number of classes, and testing performance drops while using datasets that have more classes \textcolor{red}{(add citation here, the survey should be good)}. As far as we know, no work on Open-Set Recognition has been done on a dataset with 335 ImageNet classes, which indicates that current methods may only apply to smaller datasets, and may not generalize well with bigger datasets.
    
    \item \textbf{Input Image Size for Deep Learning Based Models: } As mentioned above, most of the datasets used for Open-Set research only contains a small number of classes; besides, the image sizes from these datasets are usually one of the follows: 16x16, 32x32 and 64x64; and none of them has an image size of 224x224, which is the input size of out model.
    
    Considering we reproduce these baselines to make basic comparisons, heavily tuning parameters from these baselines, modifying the methods, or re-implementing the methods from scratch to improve performance is against our purpose. Besides, some methods contain generative networks for synthesizing data, and it cost much more time and computational resource to generate images of size 224x224. To be able to use our data, we have to downsize our input image to match the input size required by each method, which potentially lead to heavy loss of information during training phase. 
    
    \item \textbf{Feature Space Size for SVM Based methods: } As we mention in \textcolor{red}{(add section here)}, we have to use PCA to reduce the size of features for a few methods, including: SVM. W-SWM, Pi-SVM and EVM. The reduced features guarantee these algorithms finish running in a reasonablemap amount of time, but are also much smaller in size \textcolor{red}{(Add feature size here: before and after PCA. Other things to consider: does reducing feature size lead to worse performance? Or maybe the model is already bad even before PCA - but we don't know about this, because we can't run these methods on original features.)}
    
    \item \textbf{Others: } \textcolor{red}{(We found out that there is a flaw in the design of OpenMax. OpenMax uses the features that are predicted correctly to calculate MAV, distances and so on, but it is possible that no sample in a class is predicted correctly, if a dataset is complex/difficult.)}
\end{itemize}


==> Arxiv submission file/sections/g_conclusion.tex <==
\section{Discussion and Future Work}

% Snipped for space. -WJS.
%We described a new method for improving OSR performance using measurements of human perception. Specifically, we examined a training regime for machine learning that incorporated a psychophysical loss function and a network architecture that supported variable RT measurements to enforce biological fidelity in the processing time of input images. Experiments showed that by adding an additional information stream  --- human RT associated with the recognition of known samples --- the resulting model generalized better in object recognition settings where limited training data and a large amount of novelty were present. 

While our method is applied to a limited number of training samples in this study, it is also possible to utilize the psychophysical loss function on larger datasets (including those with outlier samples~\cite{Deep_Anomaly_Detection_with_Outlier_Exposure}). We argue that human RT can still improve model performance, because it provides extra information for deciding whether a sample should be known or unknown. It is worth mentioning that with a larger training dataset, a larger number of RT measurements may be necessary. Limitations for the proposed method are focused around the data collection. For instance, if a large amount of human data is required then the data collection process can be very time consuming. Further, the collected human data is task specific, and is difficult to transfer to other applications. However, these are opportunities for future work.

Turning to humans as a reference point for OSR problems is a promising new direction of work, and our results hint at the potential other experimental practices from the field of psychology might have in providing information beyond simple labels to supervised learning. 
Gaze measurement has already been suggested as one data stream~\cite{zhang2018agil}. 
More intriguing though is the measurement of pupil dynamics. A recent study has shown that movement of the pupil can be used as an index of mental effort exertion~\cite{pupil}, and thus could be another indicator of the patterns of error in training data.

There is also work that looks at the relationship between human behavior and machine learning models beyond RT, suggesting that human perception does not always align with model decisions. Geirhos et al.~\cite{Generalisation_in_humans} suggest that humans and computer vision models process information in different ways, and Kotseruba et al.~\cite{saliency_model} argue that training CNNs with psychophysical data does not improve the performance of saliency models. 
This research provides a foundation for exploring what types of tasks can benefit from psychophysics and alternative ways to incorporate human behavior into  algorithms. With RT, we are just scratching the surface.

% \textcolor{red}{Should we talk about the limitations of the paper/method?}

%In this paper, we introduce a large-scale data collection on human reaction time, and a novel loss function that utilizes these reaction time entries to train MSD-Net for Open-Set Recognition task on our dataset. Thorough experiments and evaluation show that our new formulation achieve best performance among all 11 methods on testing both known and unknown class. Our method also shows simplicity in implementation and training, and does not require much fine tuning. Although numerous works have been proposed for Open-Set problem in recent years, handling Open-Set with deep network still remains a great challenge; how to gain better features and to determine decision boundary to distinguish known and unknown require much dedication and exploration. 
%Based on this work, it is possible to explore more possibilities on using human biology knowledge for multiple tasks. 
%For example, human reaction time could be used in other domains that contain novelty and not restricted to natural images from ImageNet, including hand writing characters, cartoon images or video game inputs; this could also possibly be applied to activity recognition.
%Another domain that may benefit from human perception input is biometrics.
%For instance, human pupil and iris information could be used as an index of effort exertion \cite{pupil}; by collecting human data on pupils, it could be possible to build models to analyze how much effort people are putting into a task.
%Besides, we also look forward to seeing more evaluation strategies and more complex datasets be developed for Open-Set Recognition.

%and we address that previous methods that work well with common standard datasets may fail on more complex datasets. As far as we known, this is the first study that utilizes human data to improve Open-Set Recognition and our work proposes a brand-new idea for tackling Open-Set problem with human biologically-inspired methods. Our work is also the very first to use a larger dataset for Open-Set, comparing to the traditional datasets used in other baselines. With our psychophysical loss, we are able to train a network with only 33548 known samples from 293 class in ImageNet. Thorough experiments and evaluation show that our new formulation achieve best performance among all 11 methods, on testing 336453 known samples from the same 293 classes and 48067 samples from 42 ImageNet classes as one unknown class. Our method also shows simplicity in implementation and training, and does not require much fine tuning. 


==> README <==

August 26, 2015


IEEEtran is a LaTeX class for authors of the Institute of Electrical and
Electronics Engineers (IEEE) transactions journals and conferences.
The latest version of the IEEEtran package can be found at CTAN:

http://www.ctan.org/pkg/ieeetran

as well as within IEEE's site:

http://www.ieee.org/


This package contains the IEEE Computer Society subset of the full IEEEtran
package and is intended for use with IEEE Computer Society publications.
The included version of the IEEEtran_HOWTO.pdf has been specially formatted
in IEEE Computer Society (compsoc) journal mode.


For latest news, helpful tips, answers to frequently asked questions,
beta releases and other support, visit the IEEEtran home page at my
website:

http://www.michaelshell.org/tex/ieeetran/

Version 1.8b has a number of significant changes over the v1.8a release.
For a full history of changes, please read the file changelog.txt.
The most notable changes in this release include:

 1) Added new comsoc mode for the IEEE Communications Society.
    This mode (at present) only invokes the use of the newtxmath math fonts.
 
 2) Revised IEEEeqnarray column specifications to work with active " 
    (or other punctuation catcode changes) as with babel under the
    german or ngerman language modes. 
    Thanks to Stefan M. Moser for reporting this problem.

 3) Added \indexspace and other index related macros as newer versions of
    article.cls now do. These macros are needed to avoid an error when
    using the glossaries package.
    Thanks to Sebastian Nyberg for suggesting this change.

 4) Fixed odd/even page header font bug under compsoc mode and
    other page style code improvements.
    Thanks to Marco Paolieri for reporting this problem.

 5) Added hooks to allow for easy control of spacing above title.

 6) Added the \IEEEnoauxwrite command.
    Thanks to Sudarshan Mukherjee for suggesting this feature.


NOTE: Take care not to confuse the "comsoc" and "compsoc" class
options/modes as they are very different:

comsoc  ==> IEEE Communications Society
compsoc ==> IEEE Computer Society

The comsoc mode requires that an acceptable Times math font be available on
the LaTeX system. This requirement will be enforced by IEEEtran in comsoc
mode. Either the freely available newtxmath font by Michael Sharpe
http://www.ctan.org/pkg/newtx
(version 1.451, July 28, 2015 or later is recommended)
or the commercial MathTime font (e.g., mtpro2.sty) is acceptable.
See Section II-D (2.4) "Class Options - comsoc, compsoc, transmag" of
the IEEEtran HOWTO for more details.


Best wishes for all your publication endeavors,

Michael Shell
http://www.michaelshell.org/


********************************** Files **********************************

README                 - This file.

IEEEtran.cls           - The IEEEtran LaTeX class file.

changelog.txt          - The revision history.

IEEEtran_HOWTO.pdf     - The IEEEtran LaTeX class user manual.

bare_conf_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         conference papers.

bare_jrnl_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         journal papers.

bare_adv.tex           - A bare bones starter file showing advanced
                         techniques such as conditional compilation,
                         hyperlinks, PDF thumbnails, etc. The illustrated
                         format is for a IEEE Computer Society journal paper.

***************************************************************************
Legal Notice:
This code is offered as-is without any warranty either expressed or
implied; without even the implied warranty of MERCHANTABILITY or
FITNESS FOR A PARTICULAR PURPOSE! 
User assumes all risk.
In no event shall the IEEE or any contributor to this code be liable for
any damages or losses, including, but not limited to, incidental,
consequential, or any other damages, resulting from the use or misuse
of any information contained here.

All comments are the opinions of their respective authors and are not
necessarily endorsed by the IEEE.

This work is distributed under the LaTeX Project Public License (LPPL)
( http://www.latex-project.org/ ) version 1.3, and may be freely used,
distributed and modified. A copy of the LPPL, version 1.3, is included
in the base LaTeX documentation of all distributions of LaTeX released
2003/12/01 or later.
Retain all contribution notices and credits.
** Modified files should be clearly indicated as such, including  **
** renaming them and changing author support contact information. **

File list of work: IEEEtran.cls, IEEEtran_HOWTO.pdf, bare_adv.tex,
                   bare_conf_compsoc.tex, bare_jrnl_compsoc.tex.
***************************************************************************


==> sections/f_discussion.tex <==
\section{Discussion}

Table \ref{tab:all_results} shows testing results on known samples and unknown samples for all methods including model trained with our psychophysical loss, and the bold number in each column indicates the method that has the best performance on that metric.

While most of the methods only achieve a performance that is only a little better than making a random choice among 293 known class, Cross-Entropy, Cross-Entropy with performance loss and psyphy model maintain excellent top-1 accuracy on testing on known samples. EVM has the highest accuracy when tested with unknown samples, but when we look at other metrics all together, we notice that it tends to classify everything as unknown. Similar with EVM, CROSR and CAC-OSR also classify most of the samples as unknown, leading to a high accuracy on testing unknown, but a high number of false positive. On the other hand, OSRCI classifies most of the classes as known, which indicates it produces high probability scores for both known and unknown samples, and it is not able to distinguish known and unknown. SVM and OpenMax are more balanced when it comes to Open-Set Recognition and produce decent accuracy score while tested with unknown samples, and they also both generate good F-1 scores; but like other algorithms, they failed to perform well on the closed-set part to classify known samples into a correct class. Only the last 3 methods shown in the table are able to maintain good performance on testing known samples, and distinguish unknown from known at the same time; and overall, our psyphy model achieves highest performance on testing top-1 accuracy, F1-score and MCC.

We look more closely into each method and the result we have to analyze the reasons why some methods failed on the task.

\textcolor{red}{I feel we should mention why we used fixed threshold? Where to put it}

\begin{itemize}
    \item \textbf{Dataset Size: } Most of the Open-Set Recognition papers utilize a few standard datasets, including but not limited to LETTER (26 classes), PENDIGITS (10 classes), COIL20 (20 classes), MNIST (10 classes), SVHN (10 classes), CIFAR-10 (10 classes), CIFAR-50 (50 classes) \textcolor{red}{(need to double check this one)} and Tiny-ImageNet (200) classes. Most of these datasets do not contain a large number of classes, and testing performance drops while using datasets that have more classes \textcolor{red}{(add citation here, the survey should be good)}. As far as we know, no work on Open-Set Recognition has been done on a dataset with 335 ImageNet classes, which indicates that current methods may only apply to smaller datasets, and may not generalize well with bigger datasets.
    
    \item \textbf{Input Image Size for Deep Learning Based Models: } As mentioned above, most of the datasets used for Open-Set research only contains a small number of classes; besides, the image sizes from these datasets are usually one of the follows: 16x16, 32x32 and 64x64; and none of them has an image size of 224x224, which is the input size of out model.
    
    Considering we reproduce these baselines to make basic comparisons, heavily tuning parameters from these baselines, modifying the methods, or re-implementing the methods from scratch to improve performance is against our purpose. Besides, some methods contain generative networks for synthesizing data, and it cost much more time and computational resource to generate images of size 224x224. To be able to use our data, we have to downsize our input image to match the input size required by each method, which potentially lead to heavy loss of information during training phase. 
    
    \item \textbf{Feature Space Size for SVM Based methods: } As we mention in \textcolor{red}{(add section here)}, we have to use PCA to reduce the size of features for a few methods, including: SVM. W-SWM, Pi-SVM and EVM. The reduced features guarantee these algorithms finish running in a reasonablemap amount of time, but are also much smaller in size \textcolor{red}{(Add feature size here: before and after PCA. Other things to consider: does reducing feature size lead to worse performance? Or maybe the model is already bad even before PCA - but we don't know about this, because we can't run these methods on original features.)}
    
    \item \textbf{Others: } \textcolor{red}{(We found out that there is a flaw in the design of OpenMax. OpenMax uses the features that are predicted correctly to calculate MAV, distances and so on, but it is possible that no sample in a class is predicted correctly, if a dataset is complex/difficult.)}
\end{itemize}

